Mapping indefinite causal order processes to composable quantum protocols in a spacetime

Formalisms for higher order quantum processes provide a theoretical formalisation of quantum processes where the order of agents' operations need not be definite and acyclic, but may be subject to quantum superpositions. This has led to the concept of indefinite causal structures (ICS) which have garnered much interest. However, the interface between these information-theoretic approaches and spatiotemporal notions of causality is less understood, and questions relating to the physical realisability of ICS in a spatiotemporal context persist despite progress in their information-theoretic characterisation. Further, previous work suggests that composition of processes is not so straightforward in ICS frameworks, which raises the question of how this connects with the observed composability of physical experiments in spacetime. To address these points, we compare the formalism of quantum circuits with quantum control of causal order (QC-QC), which models an interesting class of ICS processes, with that of causal boxes, which models composable quantum information protocols in spacetime. We incorporate the set-up assumptions of the QC-QC framework into the spatiotemporal perspective and show that every QC-QC can be mapped to a causal box that satisfies these set up assumptions and acts on a Fock space while reproducing the QC-QC's behaviour in a relevant subspace defined by the assumptions. Using a recently introduced concept of fine-graining, we show that the causal box corresponds to a fine-graining of the QC-QC, which unravels the original ICS of the QC-QC into a set of quantum operations with a well-defined and acyclic causal order, compatible with the spacetime structure. Our results also clarify how the composability of physical experiments is recovered, while highlighting the essential role of relativistic causality and the Fock space structure.

==> macros.tex <==

% This package provides several macros for Quantum Information Theory, example boxes, prettifying in general 

% Adapted from Marco Tomamichel's 2011 macros by Lidia del Rio 2014, Christopher Portmann, Nuriya Nurgalieva, V. Vilasini (2017-2021).


% language input
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[T1]{fontenc}
\usepackage{afterpage}
%\usepackage{ntheorem}
\usepackage{natbib}

\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{graphicx}
\usepackage[ colorlinks = true, 
             linkcolor = MidnightBlue,
             urlcolor  = MidnightBlue,
             citecolor = orange,
             anchorcolor = ForestGreen,
]{hyperref} 
\usepackage{float}

\makeatletter
\def\mathcolor#1#{\@mathcolor{#1}}
\def\@mathcolor#1#2#3{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}
\makeatother

% additional fonts
\usepackage[sans]{dsfont} % contains font for identity character
\usepackage{bbm}
\usepackage[mathscr]{euscript}
\usepackage{cancel} %to strike out things
\usepackage{amsfonts}


%boxes and theorems
\usepackage{tcolorbox}
\tcbuselibrary{theorems} 

% more stuff
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{units}
\usepackage{framed}
\usepackage{mdframed}
\usepackage{thmtools, thm-restate} %pretty  and restatable theorems
\usepackage{ucs}
\usepackage{subcaption}
\usepackage{fullpage}
\usepackage{csquotes}
\usepackage{epigraph}


%break into cloumns
\usepackage{multicol}
\setlength{\columnsep}{0.5cm}

%enumerate in line
\usepackage{enumerate}
%\usepackage[inline]{enumitem}

% modified by Vilasini
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  tikz arrows, commutative diagrams, decorations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%tikz
\usepackage{tikz}
\usetikzlibrary{arrows}
\usepackage{rotating, xcolor}
\usetikzlibrary{shapes}
\usetikzlibrary{hobby}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{calc,intersections,through,backgrounds}
\usetikzlibrary{decorations.pathreplacing,angles,quotes}
\usetikzlibrary{arrows,decorations.markings}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{snakes} 
\usepackage{tikz-cd}
\tikzset{degil/.style={
            decoration={markings,
            mark= at position 0.5 with {
                  \node[transform shape] (tempnode) {$\setminus$};
                  %\draw[thick] (tempnode.north east) -- (tempnode.south west);
                  }
              },
              postaction={decorate}
}
}


%caption
\captionsetup[subfigure]{skip=5pt}
\captionsetup[figure]{skip=10pt}
\captionsetup[subfigure]{justification=centering}



% .......................... boxes ...........


%default colours
\tcbset{colback=orange!5,colframe=orange!75!yellow, 
%colbacktitle=orange!65!white, 
fonttitle= \bfseries, float=htb}



%..................................................

% Colours
	\newcommand{\red}[1]{\textcolor{Red}{#1}}
	\newcommand{\blue}[1]{\textcolor{Blue}{#1}}
	\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
	\newcommand{\pink}[1]{\textcolor{Magenta}{#1}}
	\newcommand{\yellow}[1]{\textcolor{Yellow}{#1}}
	\newcommand{\orange}[1]{\textcolor{Orange}{#1}}
	
 

\DeclareMathOperator{\tr}{tr}
\newcommand{\C}{\mathcal}



%comments
\newcommand{\ms}[1]{\textcolor{black!60!green}{ [#1]}}
\newcommand{\vv}[1]{\textcolor{blue}{ [#1]}}
	
% Referencing equations and figures
	\newcommand{\eref}[1]{Eq.\ \ref{#1}}
	\newcommand{\fref}[1]{Fig.\ \ref{#1}}
	
	
% ........................................................
	
	
% ........... Hilbert spaces and states  ...............
	
% Dirac notation
    \newcommand{\ket}[1]{\vert  #1 \rangle}
    \newcommand{\bra}[1]{\langle #1 |}
    \newcommand{\inprod}[2]{\langle #1 | #2 \rangle}
	\newcommand{\proj}[2]{\ket{#1}\bra{#2}}
	\newcommand{\pure}[1]{\proj{#1}{#1}}
 

% Hilbert spaces
	\newcommand{\hilbert}{\mathcal{H}}
	\newcommand{\composed}{\mathcal{H}_A  \otimes \mathcal{H}_R}
	


% ..... operators and maps .....  

% Powerset
	\newcommand{\Powerset}[1]{\operatorname{Powerset}(#1)} 

% Span
	\newcommand{\Span}[1]{\operatorname{Span}(#1)} 
	
% Diagonal 
\newcommand*{\diag}{\operatorname{diag}}


%Identity operator
	\newcommand{\id}{\mathbbm{1}}
    %\newcommand{\id}{id}

% % Trace
	\newcommand{\tr}{\operatorname{Tr}  }
	\DeclareMathOperator{\Tr}{Tr}

%TPCPMs
\newcommand*{\I}{\mathcal{I}}
\newcommand*{\E}{\mathcal{E}}
\newcommand*{\cM}{\mathcal{M}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\OO}[1]{\mathcal{O} \left( #1 \right) }
% % \newcommand{\ham}{\mathcal{H}}




% ...........  general maths  .................

% % Vectors
	\renewcommand{\vec}[1]{\mathbf{#1}}
	\newcommand{\vecop}[1]{\hat{\mathbf{#1}}}


%Set
	\newcommand{\set}[1]{\left\{ #1 \right\}}


% % Absolute value
	\newcommand{\abs}[1]{\left| #1 \right|}

% Matrices
	\newcommand{\matrixTwo}[1]{
		\left( 
			\begin{array}{c c}
				#1
			\end{array}
		\right)
		}
	\newcommand{\matrixN}[2]{
		\left( 
			\begin{array}{#1}
				#2
			\end{array}
		\right)
		}

% Probability
	%\newcommand{\prob}{\mathcal{P}}
	%\newcommand{\Prob}[1]{\mbox{Prob} \left[ #1 \right]}
	% Long probabilities
	\newcommand{\prob}[2]{
		\Pr_{#1}
		\left\{
			\begin{array}{l}
				#2
			\end{array}
		\right\}
		}

% ............................................

% Little things
	\newcommand{\ie}{i.e., }
	\newcommand{\etal}{et al.\ }
	\newcommand{\cj}{Choi-Jamio\l{}kowski }
	%\newcommand{\iid}{i.i.d.\  }

	\newcommand*{\eps}{\varepsilon}
	\newcommand*{\half}{\frac{1}{2}}
    \newcommand{\Ss}{state-space }
    \newcommand{\constr}[1]{\overset{#1}{\to}}




% added by Christopher
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  multiple links to the same footnote
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\footnoteremember}[2]{\footnote{\label{#1}#2}\newcounter{#1}\setcounter{#1}{\value{footnote}}}
\newcommand{\footnoterecall}[1]{\hyperref[#1]{\footnotemark[\value{#1}]}}



% added by Nuriya, Vilasini
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  clever ref, proof
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[capitalise, noabbrev]{cleveref}
\newenvironment{proof}{\paragraph{Proof:}}{\hfill$\square$}

%\input{Qcircuit}
\usepackage[page]{totalcount}
%\usepackage{thmtools, thm-restate}

\usetikzlibrary{shapes}
\usetikzlibrary{hobby}
\usetikzlibrary{decorations.markings}

% added by Vilasini
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  theorem environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
%\declaretheorem[style=boxed]{definition}



\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1\langle}\)}%
  \mathopen{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1\rangle}\)}%
  \mathclose{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\makeatother


